Towards Open Domain Text-Driven Synthesis of Multi-Person Motions

This work aims to generate natural and diverse group motions of multiple humans from textual descriptions. While single-person text-to-motion generation is extensively studied, it remains challenging to synthesize motions for more than one or two subjects from in-the-wild prompts, mainly due to the lack of available datasets. In this work, we curate human pose and motion datasets by estimating pose information from large-scale image and video datasets. Our models use a transformer-based diffusion framework that accommodates multiple datasets with any number of subjects or frames. Experiments explore both generation of multi-person static poses and generation of multi-person motion sequences. To our knowledge, our method is the first to generate multi-subject motion sequences with high diversity and fidelity from a large variety of textual prompts.

==> tables/ablation-guidance.tex <==





 \begin{table*}[h]
    \centering
    \caption{Ablation results for different classifier-free guidance term scales. The ``1/2'' here means different scales for the first and second stage of our model.}

    \scalebox{0.9}{

    \begin{tabular}{l c c c c c c c c}
    \toprule
    \multirow{2}{*}{1/2 CFG}  
    & \multicolumn{3}{c}{P-R-Precision $\uparrow$} 
    & \multirow{2}{*}{P-FID $\downarrow$} 
    & \multirow{2}{*}{P-Sim $\uparrow$} 
    & \multirow{2}{*}{P-Div $\rightarrow$} 
    & \multirow{2}{*}{M-FID $\downarrow$} 
    & \multirow{2}{*}{M-Div $\rightarrow$} \\

    \cline{2-4}
    ~ & Top-1 & Top-2 & Top-3 \\
    
    \toprule

    
        \textbf{Data}    &
         0.621        & % top 1
         0.737        & % top 2
         0.819        & % top 3
         0.000        & % FID
         0.378        & % mm-dist
         1.366        & % diversity
         0.002        & % M-FID
         1.342        \\ % M-Div


    \midrule

    1.0/1.0        &
         0.380        & % top 1
         0.537        & % top 2
         0.626        & % top 3
         0.224        & % FID
         0.245        & % mm-dist
         1.318        & % diversity
         0.682        & % M-FID
         1.220        \\ % M-Div

    1.75/1.0        &
         0.438        & % top 1
         0.589        & % top 2
         0.672        & % top 3
         0.220        & % FID
         0.260        & % mm-dist
         1.329        & % diversity
         0.674        & % M-FID
         1.210        \\ % M-Div

    1.0/1.5        &
         0.420        & % top 1
         0.561        & % top 2
         0.647        & % top 3
         0.221        & % FID
         0.253        & % mm-dist
         1.328        & % diversity
         0.677        & % M-FID
         1.205        \\ % M-Div

    1.75/1.5        &
         0.539        & % top 1
         0.704        & % top 2
         0.776        & % top 3
         0.229        & % FID
         0.304        & % mm-dist
         1.329        & % diversity
         0.684        & % M-FID
         1.220        \\ % M-Div



    \bottomrule
    
    \end{tabular}}
    \label{tab:cfg}

\end{table*}



 \begin{table*}[h]
    \centering
    \caption{Ablation results for different pose and motion guidance term scales.}

    \scalebox{0.9}{

    \begin{tabular}{l c c c c c c c c}
    \toprule
    \multirow{2}{*}{P/M Guidance}  
    & \multicolumn{3}{c}{P-R-Precision $\uparrow$} 
    & \multirow{2}{*}{P-FID $\downarrow$} 
    & \multirow{2}{*}{P-Sim $\uparrow$} 
    & \multirow{2}{*}{P-Div $\rightarrow$} 
    & \multirow{2}{*}{M-FID $\downarrow$} 
    & \multirow{2}{*}{M-Div $\rightarrow$} \\

    \cline{2-4}
    ~ & Top-1 & Top-2 & Top-3 \\
    
    \toprule

    
        \textbf{Data}    &
         0.621        & % top 1
         0.737        & % top 2
         0.819        & % top 3
         0.000        & % FID
         0.378        & % mm-dist
         1.366        & % diversity
         0.002        & % M-FID
         1.342        \\ % M-Div


    \midrule

    0.0/0.0        &
         0.525        & % top 1
         0.685        & % top 2
         0.766        & % top 3
         0.253        & % FID
         0.297        & % mm-dist
         1.328        & % diversity
         0.687        & % M-FID
         1.204        \\ % M-Div

    0.2/0.0        &
         0.546        & % top 1
         0.696        & % top 2
         0.780        & % top 3
         0.218        & % FID
         0.303        & % mm-dist
         1.341        & % diversity
         0.673        & % M-FID
         1.231        \\ % M-Div

    0.4/0.0        &
         0.560        & % top 1
         0.723        & % top 2
         0.795        & % top 3
         0.200        & % FID
         0.310        & % mm-dist
         1.342        & % diversity
         0.683        & % M-FID
         1.234        \\ % M-Div


    0.0/0.2        &
         0.515        & % top 1
         0.677        & % top 2
         0.769        & % top 3
         0.207        & % FID
         0.300        & % mm-dist
         1.335        & % diversity
         0.700        & % M-FID
         1.207        \\ % M-Div

    0.2/0.2        &
         0.549        & % top 1
         0.710        & % top 2
         0.791        & % top 3
         0.192        & % FID
         0.307        & % mm-dist
         1.340        & % diversity
         0.713        & % M-FID
         1.220        \\ % M-Div

    0.4/0.2        &
         0.547        & % top 1
         0.713        & % top 2
         0.778        & % top 3
         0.173        & % FID
         0.309        & % mm-dist
         1.332        & % diversity
         0.706        & % M-FID
         1.211        \\ % M-Div



    0.0/0.4        &
         0.535        & % top 1
         0.694        & % top 2
         0.776        & % top 3
         0.193        & % FID
         0.354        & % mm-dist
         1.377        & % diversity
         0.727        & % M-FID
         1.229        \\ % M-Div

    0.2/0.4        &
         0.529        & % top 1
         0.702        & % top 2
         0.792        & % top 3
         0.181        & % FID
         0.354        & % mm-dist
         1.382        & % diversity
         0.715        & % M-FID
         1.210        \\ % M-Div

    0.4/0.4        &
         0.556        & % top 1
         0.718        & % top 2
         0.790        & % top 3
         0.175        & % FID
         0.315        & % mm-dist
         1.382        & % diversity
         0.736        & % M-FID
         1.118        \\ % M-Div



    \bottomrule


    
    
    \end{tabular}}
    \label{tab:ablation}

\end{table*}

